Causal Inference Under Network Interference

We review the growing body of research on the challenging topic of interference in causal inference. Interference arises when the treatment assignments of connected units affect the outcomes of other units directly (via spillover) or indirectly (via contagion). Examples include public health, economic, political, or educational interventions, as well as advertising on social media. Adapting the Neyman-Rubin potential outcome framework, we review selected causal effects under interference and discuss identification of causal effects based on experimental and observational data. We then review statistical tests for interference and causal effects, design- and model-based estimators for causal effects, and methodological challenges, including variance reduction, unknown interference graphs, and misspecified exposure mappings. We conclude with a discussion of the scope of causal conclusions based on fixed and random potential outcomes and interference graphs. While the fixed potential outcome framework is sufficient in many applications, the random potential outcome framework can be useful when the data fall short. Examples include causal inference for heterogeneous treatment effects and external validity, including generalizability and transportability.

==> capturing.contagion.tex <==
While contagion cannot be identified as a causal process based on outcomes observed at a single time point, 
contagion can be accommodated  by
\bi 
\item modeling dependence of outcomes $Y_1, \ldots, Y_N$ conditional on treatment assignments $X_1, \ldots, X_N$;
\vspace{.05cm}
\item or modeling dependence among fixed potential outcomes $y_1(\bx), \ldots, y_N(\bx)$ or random potential outcomes $Y_1(\bx), \ldots, Y_N(\bx)$ ($\bx \in \mX$).
\ei 
These two approaches are equivalent under igorability assumptions (Section \ref{sec:identification}).
In both the fixed and random potential outcome frameworks, 
there have been attempts to model dependence among potential outcomes that accommodate contagion \cite{leung2022causal,OgShLe20,TTFuSh21,BhSe24}.
These attempts may be deterministic or probabilistic,
depending on whether potential outcomes are fixed or random.

\vspace{.1cm}

\input{interference}

==> confidence.intervals.tex <==
While unbiasedness extends from fixed to random potential outcomes subject to restrictions on the set of $(\by(\cdot), \bz)$,
the coverage probabilities of confidence intervals may not.
To demonstrate,
consider any $\alpha \in (0, 1)$ and let $\mathscr{S}$ be an interval estimator of $\theta_\mX(\by(\cdot),\bz)$,
provided that $(\by(\cdot),\bz)\in\mY_s(\cdot)\times \mZ_s$.
If
\be
\label{condition00}
\mbP_{\mX\mid\mY(\cdot),\mZ}(\theta_\mX(\bY(\cdot),\bZ) \in \mathscr{S} | (\bY(\cdot),\bZ)\hspace{-0.085cm}=\hspace{-0.085cm}(\by(\cdot),\bz))\s
\\
> 1-\alpha \text{ for all $(\by(\cdot),\bz)\in \mY_s(\cdot)\times \mZ_s$,}
\ee
then
\beno
\mbP_{\mX,\mY(\cdot),\mZ}(\theta_\mX(\bY(\cdot),\bZ) \in \mathscr{S})
> 1-\alpha,
\ee
provided that $(\bY(\cdot),\bZ)$ is generated from a distribution with support contained in $\mY_s(\cdot)\times \mZ_s$.
That said,
even when the condition in Equation \eqref{condition00} is satisfied,\break % I removed "strong" because the subset $\mY_s(\cdot)\times \mZ_s$ is part of the theoretical guarantee in the fixed setting
% A researcher does not first fix a subset $\mY_s(\cdot)\times \mZ_s$ and then try to prove results for all $(\by(\cdot),\bz)\in \mY_s(\cdot)\times \mZ_s$
% Instead, they try to find a set $\mY_s(\cdot)\times \mZ_s$ for which they have guarantees for all $(\by(\cdot),\bz)\in \mY_s(\cdot)\times \mZ_s$.
% Any theoretical guarantee in the fixed setting comes with one such choice of $\mY_s(\cdot)\times \mZ_s$
% So the condition is automatically satisfied for that choice
$\mbP_{\mX,\mY(\cdot),\mZ}(\theta_{\mX,\mY(.),\mZ} \in\mathscr{S})$ may be less than $1-\alpha$,
because confidence intervals for $\theta_{\mX,\mY(\cdot),\mZ}$ will depend on the variability of $\theta_{\mX}(\bY(\cdot),\bZ)$ around its mean $\theta_{\mX,\mY(\cdot),\mZ}$.

==> doubly.robust.estimators.tex <==
A popular example is doubly robust estimators based on exposure mappings \citep{liu2019doubly,viviano2024policy,khatami2025gml,bong2025heterogeneous}.
Doubly robust estimators combine design-based estimators with model-based estimators that make assumptions about the process generating potential outcomes,
and can hence be viewed as model-based.
Let $m(d; \bm{c}_i,\bz)$ be the conditional expectation of the outcome $Y_i$ of unit $i$ given exposure level $f_i(\bX) = d$,
confounders $\bm{C}_i = \bm{c}_i$,
and interference graph $\bZ = \bz$:
\beno
m(d; \bc_i, \bz) 
&\coloneqq& \mbE_{\mY\mid\mathscr{F}_i,\mC_i,\mZ}[Y_i \mid (f_i(\bX), \bm{C}_i, \bZ) = (d, \bc_i, \bz)].
\ee
A doubly robust estimator of $\mu^E(d)$ is
\beno
\widehat\mu_{DR}^E(d)
&\coloneqq& \dfrac{1}{N} \dsum_{i=1}^N \dfrac{(Y_i - \widehat{m}(d; \bm{C}_i, \bZ))\, \mbI(f_i(\bX) = d)}{\widehat\psi(d; \bm{C}_i, \bZ)}\s
\\
&+& \dfrac{1}{N} \dsum_{i=1}^N \widehat{m}(d; \bm{C}_i, \bZ),
\ee
where $\widehat\psi(d; \bm{C}_i, \bZ)$ is an estimator of the propensity score $\psi(d; \bm{C}_i, \bZ)$ and $\widehat{m}(d; \bC_i, \bZ)$ is an estimator of the conditional expectation $m(d; \bC_i, \bZ)$ obtained by regressing the observed outcomes $Y_i$ on $(f_i(\bX), \bm{C}_i, \bZ) = (d, \bc_i, \bz)$ ($i = 1, \ldots, N$).
The estimator $\widehat\mu_{DR}^E(d)$ combines a design-based estimator $\widehat\psi(d; \bm{C}_i, \bZ)$ with a model-based estimator $\widehat{m}(d; \bC_i, \bZ)$,
which makes assumptions about the process generating potential outcomes $\bY(\cdot)$ to estimate $\widehat{m}(d; \bC_i, \bZ)$.
Its double robustness stems from the fact that if either the design-based estimator $\widehat\psi(d; \bC_i, \bZ)$ or the model-based estimator $\widehat{m}(d; \bC_i, \bZ)$ is consistent, 
then so is $\widehat\mu_{DR}^E(d)$ \citep{viviano2024policy}.

==> figure.contagion.tex <==
\begin{figure}
\vspace{-.25cm}
\begin{center}
\begin{tabular}{ccc}
      \tikz{ %
        \node[\obs] (y1) {$Y_1$} ; %
        \node[\obs, right=of y1] (y2) {$Y_2$} ; %
        \node[\obs, below=of y1, yshift=0cm] (h1) {$X_1$} ; %
        \node[\obs, below=of y2, yshift=0cm] (h2) {$X_2$} ; %
        \edge[color=black, line width=1pt]{h1} {y1} ; %
        \edge[color=MidnightBlue, line width=1.15pt]{h1} {y2} ; %
        \edge[color=black, line width=1pt]{h2} {y2} ; %
        \edge[color=MidnightBlue, line width=1pt]{h2} {y1} ; %
        \edge[color=orange, line width=1.25pt]{y1}{y2} ; %
      }
&
      \tikz{ %
        \node[\obs] (y1) {$Y_1$} ; %
        \node[\obs, right=of y1] (y2) {$Y_2$} ; %
        \node[\obs, below=of y1, yshift=0cm] (h1) {$X_1$} ; %
        \node[\obs, below=of y2, yshift=0cm] (h2) {$X_2$} ; %
        \edge[color=black, line width=1pt]{h1} {y1} ; %
        \edge[color=MidnightBlue, line width=1.15pt]{h1} {y2} ; %
        \edge[color=black, line width=1pt]{h2} {y2} ; %
        \edge[color=MidnightBlue, line width=1pt]{h2} {y1} ; %
        \edge[color=orange, line width=1.25pt]{y2}{y1} ; %
      }
& 
      \tikz{ %
        \node[\obs] (y1) {$Y_1$} ; %
        \node[\obs, right=of y1] (y2) {$Y_2$} ; %
        \node[\obs, below=of y1, yshift=0cm] (h1) {$X_1$} ; %
        \node[\obs, below=of y2, yshift=0cm] (h2) {$X_2$} ; %
        \node[\lat, above=of y1, xshift=0.85cm, yshift=-.25cm] (u) {$U$} ; %
        \edge[color=black, line width=1pt]{h1} {y1} ; %
        \edge[color=MidnightBlue, line width=1.15pt]{h1} {y2} ; %
        \edge[color=black, line width=1pt]{h2} {y2} ; %
        \edge[color=MidnightBlue, line width=1pt]{h2} {y1} ; %
        \edge[color=orange, line width=1.25pt]{u}{y1,y2} ; %
      }
\\
(a) Contagion
& (b) Contagion
& (c) Unobserved $U$:
\\
&& \hspace{.25cm} common source
\end{tabular}
\caption{\label{graph.contagion}
If $Y_1$ and $Y_2$ are observed at a single time point,
we cannot distinguish whether
(a) $Y_1$ affects $Y_2$,
(b) $Y_2$ affects $Y_1$,
or (c) the dependence between $Y_1$ and $Y_2$ conditional on $X_1$ and $X_2$ is induced by an unobserved variable $U$ that affects both $Y_1$ and $Y_2$.
As a result,
contagion cannot be identified as a causal process,
but it can be accommodated by capturing dependence between $Y_1$ and $Y_2$ conditional on $X_1$ and $X_2$.
The source of dependence in examples (a) and (b) is contagion,
whereas the source of dependence in example (c) is an unobserved variable $U$.
}
\end{center}
\end{figure}

==> figure.interference.tex <==
\begin{figure}
\begin{tabular}{cc}
      \hspace{.5cm} \mbox{}\tikz{ %
        \node[\obs] (y1) {$Y_1$} ; %
        \node[\obs, right=of y1] (y2) {$Y_2$} ; %
        \node[\obs, below=of y1, yshift=0cm] (h1) {$X_1$} ; %
        \node[\obs, below=of y2, yshift=0cm] (h2) {$X_2$} ; %
        \edge[color=black, line width=1pt]{h1} {y1} ; %
        \edge[color=black, line width=1pt]{h2} {y2} ; %
      }
& \hspace{.5cm} \mbox{}
      \tikz{ %
        \node[\obs] (y1) {$Y_1$} ; %
        \node[\obs, right=of y1] (y2) {$Y_2$} ; %
        \node[\obs, below=of y1, yshift=0cm] (h1) {$X_1$} ; %
        \node[\obs, below=of y2, yshift=0cm] (h2) {$X_2$} ; %
        \edge[color=black, line width=1pt]{h1} {y1} ; %
        \edge[color=MidnightBlue, line width=1pt]{h1} {y2} ; %
        \edge[color=black, line width=1pt]{h2} {y2} ; %
        \edge[color=MidnightBlue, line width=1pt]{h2} {y1} ; %
      }
      \\
      \hspace{.5cm}(a) \mbox{ No interference } & \hspace{.5cm}(b) \mbox{ Interference:}\\
      \hspace{.5cm}& \hspace{.85cm}\mbox{spillover}\s\\
      \hspace{.5cm} \mbox{}\tikz{ %
        \node[\obs] (y1) {$Y_1$} ; %
        \node[\obs, right=of y1] (y2) {$Y_2$} ; %
        \node[\obs, below=of y1, yshift=0cm] (h1) {$X_1$} ; %
        \node[\obs, below=of y2, yshift=0cm] (h2) {$X_2$} ; %
        \edge[color=black, line width=1pt]{h1} {y1} ; %
        \edge[color=black, line width=1pt]{h2} {y2} ; %
        \edge[-, color=orange, line width=1.25pt]{y1}{y2} ; %
      }
& \hspace{.5cm} \mbox{} 
      \tikz{ %
        \node[\obs] (y1) {$Y_1$} ; %
        \node[\obs, right=of y1] (y2) {$Y_2$} ; %
        \node[\obs, below=of y1, yshift=0cm] (h1) {$X_1$} ; %
        \node[\obs, below=of y2, yshift=0cm] (h2) {$X_2$} ; %
        \edge[color=black, line width=1pt]{h1} {y1} ; %
        \edge[color=MidnightBlue, line width=1.15pt]{h1} {y2} ; %
        \edge[color=black, line width=1pt]{h2} {y2} ; %
        \edge[color=MidnightBlue, line width=1pt]{h2} {y1} ; %
        \edge[-, color=orange, line width=1.25pt]{y1}{y2} ; %
      }
\\
\hspace{.5cm}(c) \mbox{ Interference:} & \hspace{.5cm}(d) \mbox{ Interference:} \\
\hspace{.85cm} \mbox{contagion} & \hspace{.5cm}{\mbox{spillover and contagion}} 
\end{tabular}
\caption{\label{graph.ts.os}
A graphical representation of a population with $N = 2$ units\break 
$1, 2$,
treatment assignments $X_1, X_2$,
and outcomes $Y_1, Y_2$,
with causal effects represented by directed lines and dependence represented by undirected lines.
The black- and green-colored lines represent causal effects of treatment assignments $X_1, X_2$ on outcomes $Y_1, Y_2$ due to treatment and spillover.
The orange-colored line between $Y_1$ and $Y_2$ represents dependence conditional on $X_1$ and $X_2$ induced by contagion;
note that when $Y_1$ and $Y_2$ are observed at a single time point,
contagion cannot be identified as a causal process:
see Figure \ref{graph.contagion}.
}
\end{figure}

==> finite.path.dependence.tex <==
\hide{

at least two ways:
\bi 
\item The random potential outcomes framework can accommodate indirect interference by all units connected by a finite path.
The fixed potential outcome framework can accomplish the same,
but requires an additional assumption about the decay of the strength of interference \citep{leung2022rate}. % our example also requires this, and maybe all examples will require this, else there would be too much dependence. It might be better to give the Li and Wager example of less degree restrictions
\vspace{.1cm}
\item The random potential outcome framework facilitates the study of heterogeneous treatment effects.
\ei 
We discuss these advantages in Sections \ref{sec:adv1} and \ref{sec:adv2}.

\subsubsection{Scope: Interference}
\label{sec:adv1}

We first showcase that the random potential outcome framework can accommodate indirect interference.

}

The bulk of the literature imposes the restriction that there exists an integer $d \geq 1$ (independent of $N$) such that the potential outcomes $Y_i(\bx)$ of unit $i$ only depend on the treatment assignment $x_i$ of unit $i$ and the treatment assignments $x_j$ of other units $j$ within geodesic distance $d$ of unit $i$ in an underlying interference graph;
note that the special case $d=1$ corresponds to the neighborhood exposure assumption discussed in Section \ref{assumption1}.
By contrast, 
Markov random fields \citep{rue2005gaussian,TTFuSh21} can represent more general forms of interference:
the potential outcomes $Y_i(\bx)$ of unit $i$ can depend on the treatment assignment $x_a$ of any unit $a$ who is connected to $i$ by a finite path, 
i.e., 
$a$ does not need to be within a fixed distance from $i$:

\begin{lemma}
\label{lemm}
Consider models of $\bY(\bx) \mid \bZ = \bz$ with conditional expectations of\, $Y_i(\bx) \mid (\bY_{-i}(\bx), \bZ) = (\by_{-i}, \bz)$ satisfying Equation \eqref{natural},
and scaling constants $c_{N,i,1}(\bz) \in (0, \infty)$ and $c_{N,i,2}(\bz) \coloneqq c_{N,2}(\bz) \in (0, \infty)$ satisfying $|\delta\, c_{N,2}(\bz)| < 1/\mnorm{\bz}_2$.
Then

\beno
\mbE_{\mY(\bx)\mid\mZ}[Y_i(\bx) \mid \bZ = \bz]
&= \dsum_{d=0}^\infty\, (\delta\, c_{N,2}(\bz))^d\, \sum_{a=1}^N (\bz^d)_{i,a}\s
\\
&\times\hspace{-.05cm} \left[\beta\, x_a + \gamma\, c_{N,a,1}(\bz) {\dsum_{b=1}^N\, x_b\, z_{a,b}}\right],
\ee
where $(\bz^d)_{i,a}$ counts the number of paths of length $d$ between units $i$ and $a$ in the interference graph $\bz$.
\end{lemma}

{\color{blue}

While the basic conclusion of Lemma \ref{lemm} has been reported elsewhere \citep[e.g.,][]{TTFuSh21},
we are not aware of a formal statement and proof of Lemma \ref{lemm}.
We therefore provide a short proof of Lemma \ref{lemm} in the Appendix.

}

The main assumption of Lemma \ref{lemm} is satisfied by Gaussian Markov random fields \citep{rue2005gaussian,TTFuSh21},
which capture spillover along with correlations among potential outcomes due to contagion \citep[see][]{OgShLe20,TTFuSh21}.
Lemma \ref{lemm} implies that if the expected potential outcome $\mbE_{\mY(\bx)\mid\mZ}[Y_i(\bx) \mid \bZ = \bz]$ of unit $i$ depends on the treatment assignment $x_a$ of unit $a$, 
then there exists an integer $d \geq 1$ such that 
\bi
\item either $i$ is connected to $a$ by a path of length $d$;
\vspace{.05cm}
\item or there exists a third unit $b \in \{1, \ldots, N\} \setminus \{i,\, a\}$ such that $i$ is connected to $b$ by a path of length $d$ and $b$ is connected to $a$.
\ei
In both cases there exists a finite path between $i$ and $a$ in the interference graph.
These observations suggest that some model-based approaches can capture more general forms of interference (beyond neighborhood exposure).
In the running example,
the exposure of teenagers to advertisements of designer clothes may affect friends as well as friends of friends,
and all others who are connected to exposed teenagers directly or indirectly.

{\color{blue}

\subsubsection{Scope: Heterogeneous Treatment Effects}
\label{sec:adv2}

}


==> interference.tex <==
\paragraph*{Fixed potential outcomes}

In the fixed potential outcome framework,
contagion can be accommodated by assuming that,
for all possible treatment assignments $\bx\in\mX$, 
the potential outcomes $y_i(\bx)$ of units $i$ are related by deterministic functions $g_i$ of the form
$$y_i(\bx) = g_i(\bx, \by_{-i}(\bx), \epsilon_i),$$
where $\epsilon_i$ are non-random errors.
In general, 
it is not guaranteed that there exist potential outcomes $\by(\bx) \coloneqq (y_1(\bx), \ldots, y_N(\bx))$ satisfying the above equations.
A simple example that does satisfy the above equations is the contagion model mentioned on page 4 of \citet{yu2022estimating},
which assumes that,
for all $\bx \in \mX$,
\beno
y_i(\bx) 
= \alpha_i + \beta_i\, x_i 
+ \dsum_{j \neq i}^N \delta_{i,j}\, y_j(\bx),
\ee
where $\alpha_i \in \mbR$,
$\beta_i \in \mbR$,
and $\delta_{i,j} \in \mbR$ may be interpreted as the intercept,
the main effect of treatment,
and the effect of contagion,
respectively.
If $\delta_{i,j} = 0$ for all $(i, j)$,
there is no contagion and the $N$-vector of potential outcomes $\by(\bx)$ reduces to
\beno
\label{contagion1}
\by(\bx) 
&=& \bm\alpha + \bm{B}\, \bx,
\ee
otherwise
\be
\label{contagion2}
\by(\bx)
&=& (\bI_N - \bm\Delta)^{-1}\, \bm{\alpha} + \dsum_{d=0}^{\infty} \bm\Delta^d \bm{B}\, \bx,
\ee
where the $N \times N$-matrix $\bm{B}$ contains elements $\beta_i$ on its main diagonal and elements $0$ off its main diagonal,
while the $N \times N$-matrix $\bm\Delta$ contains elements $0$ on its main diagonal and elements $\delta_{i,j}$ off its main diagonal.
\input{capturing.contagion.fixed.potential.outcomes}

\vspace{.1cm}

\paragraph*{Random potential outcomes}

In the random potential outcome framework, contagion can be captured by assuming that,
for all $\bx\in\mX$, 
the conditional distribution of $Y_i(\bx)$ depends on $\by_{-i}(\bx)$:
$$Y_i(\bx) \mid \{\bY_{-i}(\bx) = \by_{-i}(\bx)\}\;
=\; g_i(\bx, \by_{-i}(\bx),\epsilon_i),$$
where $\epsilon_i$ are random errors.
Similar to the fixed potential outcome framework,
the above assumption is not valid in general, 
and its validity requires the conditional distributions of $Y_i(\bx)$ to be consistent with a valid joint probability distribution of $\bY(\bx)\coloneqq (Y_1(\bx),\ldots,Y_N(\bx))$.
A simple example is a linear model of the form
\beno
\label{equation2}
&& Y_i(\bx) \mid \{\bY_{-i}(\bx) = \by_{-i}(\bx)\}
\s
\\
&=&\, \alpha_i + \beta_i\, x_i + \dsum_{j\neq i}^N \delta_{i,j}\, y_j(\bx) + \epsilon_i.
\ee
If the random errors $\epsilon_i$ are Gaussian, 
$\bY(\bx)$ is multivariate Gaussian under some restrictions \citep{rue2005gaussian}.

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> model_citation_influence.tex <==
% model_citation_influence.tex
%
% Copyright (C) 2010,2011 Laura Dietz
% Copyright (C) 2012 Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Citation influence model
% Cite this model as 
% Laura Dietz, Steffen Bickel, Tobias Scheffer. 
% Unsupervised Prediction of Citation Influences. 
% In: Proceedings of International Conference on Machine Learning. 2007

%\beginpgfgraphicnamed{model-citation-influence}
\begin{tikzpicture}

  % Layout the variables
  \matrix[row sep=0.5cm, column sep=1.2cm] (LDA)
  { %
    & %
    & %
    \node[latent] (gamma)  {$\gamma$} ; & %
    \node[latent] (lambda) {$\lambda$} ; & %
    \node[latent] (psi)    {$\psi$} ; %
    \\
    \\
    \node[latent] (theta)  {$\theta$} ; & %
    & %
    \node[latent] (C)      {$C$} ; & %
    \node[latent] (S)      {$S$} ; & %
    \\
    & %
    & %
    \factor       {T-f1}   {Multi} {} {}; & %
    & %
    \factor       {T-f2}   {below:Multi} {} {}; & %
    \\
    \node[latent] (T')     {$T'$} ; & %
    & %
    \node[latent] (T)      {$T$} ; & %
    \\
    \factor       {W'-f}   {Multi} {} {}; & %
    \node[latent] (phi)    {$\phi$} ; & %
    \factor       {W-f}    {Multi} {} {}; %
    \\
    \node[obs] (W')        {$W'$} ; & %
    & %
    \node[obs] (W)         {$W$} ;
    \\
  };

  % Remaining factors
  \factor[above=of T']     {T'-f}     {left:Multi} {} {}; %
  \factor[above=of theta]  {theta-f}  {left:Dir} {} {}; %
  \factor[above=of C]      {C-f}      {left:Multi} {} {}; %
  \factor[above=of S]      {S-f}      {left:Bern} {} {}; %
  \factor[above=of gamma]  {gamma-f}  {left:Dir} {} {}; %
  \factor[above=of lambda] {lambda-f} {left:Beta} {} {}; %
  \factor[above=of psi]    {psi-f}    {left:Dir} {} {}; %
  \factor[above=of phi]    {phi-f}    {left:Dir} {} {}; %

  % Hyperparameters
  \node[const, above=of theta]  (atheta)  {$\alpha_\theta$}; %
  \node[const, above=of phi]    (aphi)    {$\alpha_\phi$}; %
  \node[const, above=of gamma]  (agamma)  {$\alpha_\gamma$}; %
  \node[const, above=of lambda, xshift=-0.5cm] (alambda1)
  {$\alpha_{\lambda_\theta}$}; %
  \node[const, above=of lambda, xshift=0.5cm] (alambda2)
  {$\alpha_{\lambda_\psi}$}; %
  \node[const, above=of psi]    (apsi)    {$\alpha_\psi$}; %

  % Factor connections
  \factoredge {phi}               {W'-f}     {W'} ; %
  \factoredge {phi}               {W-f}      {W} ; %
  \factoredge {theta}             {T'-f}     {T'} ; %
  \factoredge {theta}             {T-f1}     {T} ; %
  \factoredge {psi}               {T-f2}     {T} ; %
  \factoredge {atheta}            {theta-f}  {theta} ; %
  \factoredge {gamma}             {C-f}      {C} ; %
  \factoredge {lambda}            {S-f}      {S} ; %
  \factoredge {agamma}            {gamma-f}  {gamma} ; %
  \factoredge {alambda1,alambda2} {lambda-f} {lambda} ; %
  \factoredge {apsi}              {psi-f}    {psi} ; %
  \factoredge {aphi}              {phi-f}    {phi} ; %

  % Gates
  \gate {W'-gate} {(W'-f)(W'-f-caption)} {T'} ; %
  \gate {W-gate}  {(W-f)(W-f-caption)}   {T} ; %
  \gate {T-gate}  {(T-f1)(T-f1-caption)} {C} ;
  \vgate {T-vgate} %
  {(T-gate)} {$S=0$} %
  {(T-f2)(T-f2-caption)} {$S=1$} %
  {S} ; %

  % Plates
  \plate {LDA1} { %
    (T')(T'-f)(T'-f-caption) %
    (W')(W'-gate) %
  } {$\forall w' \in c$} ; %

  \plate {LDA2} { %
    (LDA1) %
    (theta)(theta-f)(theta-f-caption) %
  } {$\forall c \in \mathcal{C}$} ; %

  \plate {} { %
    (phi)(phi-f)(phi-f-caption) %
  } {$\forall t \in \mathcal{T}$} ; %

  \plate {P1} { %
    (W)(W-gate) %
    (T)(T-vgate) %
    (C)(C-f)(C-f-caption) %
    (S)(S-f)(S-f-caption) %
  } {$\forall w \in d$} ;

  \plate {} { %
    (P1) %
    (gamma)(gamma-f)(gamma-f-caption) %
    (lambda)(lambda-f)(lambda-f-caption) %
    (psi)(psi-f)(psi-f-caption) %
  } {$\forall d \in \mathcal{D}$} ; %

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 


==> model_lda.tex <==
% model_lda.tex
%
% Copyright (C) 2010,2011 Laura Dietz
% Copyright (C) 2012 Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Latent Diriclet allocation model

%\beginpgfgraphicnamed{model-lda}
\begin{tikzpicture}[x=1.7cm,y=1.8cm]

  % Nodes

  \node[obs]                   (X)      {$X$} ; %
  \node[latent, above=of X]    (T)      {$T$} ; %
  \node[latent, above=of T]    (theta)  {$\theta$}; %
  \node[const, above=of theta] (atheta) {$\alpha_\theta$};


  % Factors
  \factor[above=of X]     {X-f}     {Multi} {} {} ; %
  \factor[above=of T]     {T-f}     {left:Multi} {} {} ; %
  \factor[above=of theta] {theta-f} {left:Dir} {} {} ; %

  % More nodes
  \node[latent, right=of X-f] (phi)  {$\phi$}; %
  \node[const, above=of phi]  (aphi) {$\alpha_\phi$}; %

  \factor[above=of phi] {phi-f} {right:Dir} {} {} ; %

  \factoredge {theta}  {T-f}     {T} ; %
  \factoredge {atheta} {theta-f} {theta} ; %
  \factoredge {phi}    {X-f}     {X} ; %
  \factoredge {aphi}   {phi-f}   {phi} ; %

  \gate {X-gate} {(X-f)(X-f-caption)} {T}

  \plate {plate1} { %
    (X)(X-gate) %
    (T)(T-f)(T-f-caption) %
  } {$\forall 1 \leq i \leq n_d$}; %
  \plate {} { %
    (plate1) %
    (theta)(theta-f)(theta-f-caption) %
  } {$\forall d \in \mathcal{D}$} ; %
  \plate {} { %
    (phi)(phi-f)(phi-f-caption) %
  } {$\forall t \in \mathcal{T}$} ; %

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 


==> model_pca.tex <==
% model_pca.tex
%
% Copyright (C) 2012 Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% PCA model

%\beginpgfgraphicnamed{model-pca}
\begin{tikzpicture}

  % Define nodes
  \node[obs]                               (y) {$y$};
  \node[latent, above=of y, xshift=-1.2cm] (w) {$\mathbf{w}$};
  \node[latent, above=of y, xshift=1.2cm]  (x) {$\mathbf{x}$};
  \node[latent, right=2cm of y]            (t) {$\tau$};

  % Connect the nodes
  \edge {x,w,t} {y} ; %

  % Plates
  \plate {yx} {(x)(y)} {$N$} ;
  \plate {} {(w)(y)(yx.north west)(yx.south west)} {$M$} ;

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 


==> model_pca2.tex <==
% model_pca2.tex
%
% Copyright (C) 2010,2011 Laura Dietz
% Copyright (C) 2012 Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% PCA model

%\beginpgfgraphicnamed{model-pca}
\begin{tikzpicture}

  % Define nodes

  % Y
  \node[obs]          (y)   {$y$}; %
  \factor[above=of y] {y-f} {left:$\mathcal{N}$} {} {} ; %

  % W and X
  \node[det, above=of y]            (dot) {dot} ; % 
  \node[latent, above left=1.2 of dot]  (w)   {$\mathbf{w}$}; %
  \node[latent, above right=1.2 of dot] (x)   {$\mathbf{x}$}; %

  % W hyperparameters
  \node[const, above=1.2 of w, xshift=-0.5cm] (mw) {$\mu_w$} ; %
  \node[const, above=1.2 of w, xshift=0.5cm]  (aw) {$\alpha_w$} ; %

  % X hyperparameters
  \node[const, above=1.2 of x, xshift=-0.5cm] (mx) {$\mu_x$} ; %
  \node[const, above=1.2 of x, xshift=0.5cm]  (ax) {$\alpha_x$} ; %

  % noise
  \node[latent, right=2.5cm of y-f]         (t)   {$\tau$}; %
  \node[const, above=of t, xshift=-0.5cm] (at)  {$\alpha_\tau$} ; %
  \node[const, above=of t, xshift=0.5cm]  (bt)  {$\beta_\tau$} ; %

  % Factors
  \factor[above=of w] {w-f} {left:$\mathcal{N}$} {mw,aw} {w} ; %
  \factor[above=of x] {x-f} {left:$\mathcal{N}$} {mx,ax} {x} ; %
  \factor[above=of t] {t-f} {left:$\mathcal{G}$} {at,bt} {t} ; %
  \factoredge {dot,t} {y-f} {y} ; %

  % Connect w and x to the dot node
  \edge[-] {w,x} {dot} ;

  % Plates
  \plate {yx} { %
    (y)(y-f)(y-f-caption) %
    (x)(x-f)(x-f-caption) %
    (dot) %
  } {$N$} ;
  \plate {} {%
    (y)(y-f)(y-f-caption) %
    (w)(w-f)(w-f-caption) %
    (dot) %
    (yx.north west)(yx.south west) %
  } {$M$} ;

\end{tikzpicture}
%\endpgfgraphicnamed

%%% Local Variables: 
%%% mode: tex-pdf
%%% TeX-master: "example"
%%% End: 



==> nsf.preamble.tex <==
\usepackage[mathscr]{eucal}
%\newcommand\orth{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\newcommand{\Cross}{\mathbin{\tikz [x=2ex,y=2ex,line width=.2ex] \draw (0,0) -- (1,1) (0,1) -- (1,0);}}%
%\usepackage[rmx]{kpfonts}
\usepackage{dlfltxbcodetips,bbm,mathtools,subfigure,amsfonts,amsmath,amssymb,fancybox,graphicx,bm,latexsym}
% \usepackage[usenames,dvipsnames]{color}
%\newcommand{\deff}{\mathop{=}\limits^{\mbox{\tiny def}}}
%\DeclareMathOperator*{\argsup}{arg\,sup}

\newcommand{\mUTA}{\mathscr{C}}
\newcommand{\Mcle}{\widehat{\bm\Theta}(\delta)}
\newcommand{\mcle}{\widehat{\bm\theta}}

\usepackage{tikz}
\usetikzlibrary{bayesnet}
\usetikzlibrary{fit,positioning}
\newcommand{\obs}{latent}
\newcommand{\lat}{obs}
\newcommand{\alphaz}{\alpha_{\mZ,i,j}}
\newcommand{\alphaxi}{\alpha_{\mX,i}}
\newcommand{\alphaxj}{\alpha_{\mX,j}}
\newcommand{\alphay}{\alpha_{\mY,i}}
\newcommand{\alphayi}{\alpha_{\mY,i}}
\newcommand{\alphayj}{\alpha_{\mY,j}}
\newcommand{\betaxy}{\beta_{\mX,\mY,i,j}}
\newcommand{\betaxz}{\beta_{\mX,\mZ,i,j}}
\newcommand{\betayz}{\beta_{\mY,\mZ,i,j}}
\newcommand{\betaxyz}{\beta_{\mX,\mY,\mZ,i,j}}
\newcommand{\betaz}{\beta_{\mZ,\mZ,i,j}}
%\newcommand{\alphax}{\alpha_{\mY \rightarrow \mX}}
%\newcommand{\alphay}{\alpha_{\mX \rightarrow \mY}}

%\newcommand{\mP}{\mathscr{P}}
\newcommand{\wx}{\widehat{X}}
\newcommand{\att}{\bctakecare}
\newcommand{\uu}{y_1}
\newcommand{\vv}{y_2}
%\newcommand{\tv}{{\tiny\mbox{TV}}}

\usepackage[tikz]{bclogo}

\newcommand{\bt}{\begin{bclogo}[couleur={rgb:orange,0;yellow,0;white,1},arrondi=0.1,logo=\bcplume,ombre=true]}
\newcommand{\et}{\end{bclogo}\s}
\newcommand{\btt}{\begin{box}}
\newcommand{\ett}{\end{box}}

\newcommand{\btheorem}{\begin{bclogo}[couleur={rgb:orange,0;yellow,0;white,1},arrondi=0.1,logo=\bcplume,ombre=true]{Theorem}}
\newcommand{\ettheorem}{\end{bclogo}}

\newcommand{\bsh}{\begin{bclogo}[couleur={rgb:orange,0;yellow,0;white,1},arrondi=0.1,logo=\bcpanchant,ombre=true]}
\newcommand{\esh}{\end{bclogo}}

\newcommand{\wrt}{&\mbox{wrt}&}
\newcommand{\define}{\mathop{=}\limits^{\mbox{\tiny def}}}
\renewcommand{\forall}{&\mbox{for all}&}
\newcommand{\all}{&\mbox{for all}&}
\newcommand{\andd}{&\mbox{and}&}

%\usepackage[pdftex,breaklinks]{hyperref}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\inter}{\mbox{int}}
\newcommand{\benum}{\begin{enumerate}}
\newcommand{\eenum}{\end{enumerate}}

\newcommand{\llll}{\left(}
\newcommand{\rrrr}{\right)}
\newcommand{\ann}{\mbox{and}}
\newcommand{\for}{\mbox{for all}}
\newcommand{\tends}{\longrightarrow}
\newcommand{\tend}{\rightarrow}
\newcommand{\bq}{\begin{quote}\em}
\newcommand{\eq}{\end{quote}}
\newcommand{\bbq}{\begin{quote}\bf\em}
\newcommand{\ebq}{\end{quote}}
%\newcommand{\law}{\mathop{\longrightarrow}\limits^{\mbox{\footnotesize $\mathscr{L}$}}}
\newcommand{\law}{\mathop{\longrightarrow}\limits^{\mbox{\footnotesize d}}}
\newcommand{\ip}{\mathop{\longrightarrow}\limits^{\mbox{\footnotesize p}}}
\newcommand{\as}{\mathop{\longrightarrow}\limits^{\mbox{\footnotesize a.s.}}}
\newcommand{\ind}{\msim\limits^{\mbox{\tiny ind}}}
\newcommand{\iid}{\msim\limits^{\mbox{\tiny iid}}}
\newcommand{\spss}{\mathop{\longrightarrow}\limits^{\mbox{\footnotesize $N\to\infty$}}}
\renewcommand{\bar}{\overline}
\renewcommand{\=}{&=&}
\newcommand{\less}{&<&}
\newcommand{\lte}{&\leq&}
\newcommand{\gte}{&\geq&}
\newcommand{\mR}{\mathbb{R}}
\newcommand{\mK}{\mathscr{K}}
\newcommand{\mbR}{\mathbb{R}}
\newcommand{\mbN}{\mathbb{N}}
\newcommand{\mbX}{\mathbb{X}}
\newcommand{\mbA}{\mathbb{A}}
\newcommand{\one}{\mathbbm{1}}
\newcommand{\mbI}{\mathbb{I}}
\newcommand{\mbB}{\mathbb{B}}
\newcommand{\mbE}{\mathbb{E}}
\newcommand{\mbC}{\mathbb{C}}
\newcommand{\mbM}{\mathbb{M}}
\newcommand{\mbZ}{\mathcal{Z}}
\newcommand{\mbY}{\mathcal{Y}}
\newcommand{\mbS}{\mathbb{S}}
\newcommand{\mbP}{\mathbb{P}}
\newcommand{\mbQ}{\mathbb{Q}}
\newcommand{\mcO}{\mathcal{O}}
\newcommand{\mcN}{\mathscr{N}}
\newcommand{\ase}{& \mathop{\widehat{=}} &}
%\newcommand{\hide}[1]{}
%\newcommand{\ghost}[1]{}
%short version:
%\newcommand{\ghost}{.}\newcommand{\longversion}[1]{}
%long version:
%\newcommand{\ghost}{}\newcommand{\longversion}{}
\newcommand{\ba}{\begin{array}{llllllllll}}
\newcommand{\ea}{\end{array}}
\newcommand{\bea}{\begin{equation}\begin{array}{llllllllll}}
\newcommand{\eea}{\end{array}\end{equation}}
\newcommand{\nat}{\btheta}
\newcommand{\Nat}{\bTheta}
\newcommand{\truth}{\nat^\star}
\newcommand{\mple}{\widetilde\nat_{PL}}
\newcommand{\Mple}{\widetilde\Nat_{PL}}

\newcommand{\logit}{\mbox{logit}}
\newcommand{\beno}{\begin{equation}\begin{array}{llllllllll}\nonumber}
\newcommand{\be}{\begin{equation}\begin{array}{llllllllll}}
\newcommand{\ee}{\end{array}\end{equation}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\alert}{\textcolor{red}}
\newcommand{\blues}{\color{black}}
\newcommand{\alertm}{\textcolor{blue}}
\newcommand{\dis}{\displaystyle}
\newcommand{\dsum}{\displaystyle\sum\limits}
\newcommand{\dint}{\displaystyle\int\limits}
\newcommand{\dprod}{\displaystyle\prod\limits}
\newcommand{\dd}{\mathop{\mbox{d}}\nolimits}
\newcommand{\gradient}{\mathop{\nabla}\nolimits}
\newcommand{\mM}{\mbox{$\mathscr{M}$}}
\newcommand{\mN}{\mathscr{N}}
%\newcommand{\mS}{\mathscr{S}}
\newcommand{\mmS}{\footnotesize\mS_K}
\newcommand{\mG}{\mathbb{G}}
\newcommand{\mA}{\mathscr{A}}
\newcommand{\mV}{\mathscr{V}}
\newcommand{\mE}{\mathscr{E}}
\newcommand{\s}{\vspace{0.25cm}}
\newcommand{\bx}{\bm{x}}
\newcommand{\bvij}{\bm{v}_{\minusij}}
\newcommand{\bw}{\bm{w}}
\newcommand{\baa}{\bm{a}}
\newcommand{\bA}{\bm{A}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bv}{\bm{v}}
\newcommand{\bT}{\bm{T}}
\newcommand{\bX}{\bm{X}}
\newcommand{\mX}{\mathscr{X}}
\newcommand{\mT}{\mathscr{T}}
\newcommand{\mC}{\mathscr{C}}
\newcommand{\mY}{\mathscr{Y}}
\newcommand{\mI}{\mathbb{I}}
\newcommand{\mZ}{\mathscr{Z}}
\newcommand{\mD}{\mathscr{D}}
\newcommand{\mB}{\mathscr{B}}
\newcommand{\bY}{\bm{Y}}
\newcommand{\bC}{\bm{C}}
\newcommand{\bc}{\bm{c}}
\newcommand{\bbY}{\mathscr{Y}}
\newcommand{\by}{\bm{y}}
\newcommand{\bd}{\bm{d}}
\newcommand{\bu}{\bm{u}}
\newcommand{\bD}{\bm{D}}
\newcommand{\mU}{\mathscr{U}}
\newcommand{\bU}{\bm{U}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bee}{\bm{e}}
\newcommand{\bs}{\bm{s}}
\newcommand{\bz}{\bm{z}}
\newcommand{\bZ}{\bm{Z}}
\newcommand{\bS}{\bm{S}}
\newcommand{\balpha}{\mbox{\boldmath$\alpha$}}
\newcommand{\bphi}{\mbox{\boldmath$\phi$}}
\newcommand{\bbeta}{\bm{\beta}}
\newcommand{\bgamma}{\mbox{\boldmath$\gamma$}}
\newcommand{\blambda}{\mbox{\boldmath$\lambda$}}
\newcommand{\brho}{\mbox{\boldmath$\rho$}}
\newcommand{\bmu}{\mbox{\boldmath$\mu$}}
\newcommand{\bomega}{\mbox{\boldmath$\omega$}}
\newcommand{\bSigma}{\mbox{\boldmath$\Sigma$}}
\newcommand{\bTheta}{\bm\Theta}
\newcommand{\bta}{\mbox{\boldmath$\eta$}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\hatbtheta}{\boldsymbol{\hat{\theta}}}
\newcommand{\bvartheta}{\mbox{\boldmath$\vartheta$}}
\newcommand{\bpi}{\mbox{\boldmath$\pi$}}
\newcommand{\bxi}{\mbox{\boldmath$\xi$}}
\newcommand{\bXi}{\mbox{\boldmath$\Xi$}}
\newcommand{\bpsi}{\mbox{\boldmath$\psi$}}
\newcommand{\bV}{\bm{V}}
\newcommand{\mbV}{\mathbb{V}}
\newcommand{\bLambda}{\mbox{\boldmath$\Lambda$}}
\newcommand{\bPhi}{\mbox{\boldmath$\Phi$}}
\newcommand{\bnu}{\mbox{\boldmath$\vartheta$}}
\newcommand{\vaalpha}{\vartheta_{\alpha,1}}
\newcommand{\vbalpha}{\vartheta_{\alpha,2}}
\newcommand{\vbalphaInverse}{\mbox{$\tilde{b}^{-1}_\alpha$}}
\newcommand{\vmmu}{\vartheta_{\mu,1}}
\newcommand{\vsmu}{\vartheta_{\mu,2}}
\newcommand{\vasigma}{\vartheta_{\sigma^{-2},1}}
\newcommand{\vbsigma}{\vartheta_{\sigma^{-2},2}}
\newcommand{\vbsigmaInverse}{\mbox{$\tilde{b}^{-1}_{\sigma^2}$}}
\newcommand{\bupsilon}{\mbox{\boldmath$\upsilon$}}
\newcommand{\bUpsilon}{\mbox{\boldmath$\Upsilon$}}
\newcommand{\vaVk}{\vartheta_{V_k,1}}
\newcommand{\vbVk}{\vartheta_{V_k,2}}
\newcommand{\vaVt}{\vartheta_{V_l,1}}
\newcommand{\vbVt}{\vartheta_{V_l,2}}
\newcommand{\vsthetak}{\vartheta_{\theta_k,2}}
\newcommand{\vmthetak}{\vartheta_{\theta_k,1}}
\newcommand{\vsthetal}{\vartheta_{\theta_l,2}}
\newcommand{\vmthetal}{\vartheta_{\theta_l,1}}
\newcommand{\vtaui}{\mbox{\boldmath$\vartheta_{\bm{Z_i}}$}}
\newcommand{\vtauMot}{\mbox{$\tilde{\bm{\tau}}_1$}}
\newcommand{\vtaun}{\mbox{$\tilde{\bm{\tau}}_n$}}
\newcommand{\vtauik}{\vartheta_{Z_{ik}}}
\newcommand{\vtaujl}{\vartheta_{Z_{jl}}}
\newcommand{\vtauil}{\vartheta_{Z_{il}}}
\newcommand{\vaVall}{\mbox{\boldmath$\tilde{a}_{V}$}}
\newcommand{\vbVall}{\mbox{\boldmath$\tilde{b}_{V}$}}
\newcommand{\vsthetaall}{\mbox{\boldmath$\tilde{\sigma}^2_{\theta}$}}
\newcommand{\vmthetaall}{\mbox{\boldmath$\tilde{\mu}_{\theta}$}}
\newcommand{\vtauall}{\mbox{\boldmath$\tilde{\bm{\tau}}$}}
\newcommand{\vmbeta}{\mbox{$\tilde{\mu}_{\beta}$}}
\newcommand{\vsbeta}{\mbox{$\tilde{\sigma}^2_{\beta}$}}
\newcommand{\msim}{\mathop{\rm \sim}}
\newcommand{\var}{\mathbb{V}}
%\newcommand{\var}{\mbox{Var}}
\newcommand{\cov}{\mathbb{C}}
\newcommand{\lef}{\left(}
\newcommand{\rig}{\right)}
\newcommand{\bI}{\bm{I}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bE}{\bm{E}}

\newcounter{comment}
\newenvironment{comment}[1][]{\refstepcounter{comment}\vspace{0.25cm}\par\medskip\noindent%
\textbf{Comment~\thecomment #1}:\vspace{0.25cm}\\ \rmfamily}{\medskip}
% \newcommand{\bc}{\begin{comment}\em}
% \newcommand{\ec}{\end{comment}}

%\newcounter{example}
%\newenvironment{example}[1][]{\refstepcounter{example}\par\medskip\indent%
%\textbf{Example~\theexample #1.} \rmfamily}{\medskip}

\newcounter{counterexample}
\newenvironment{counterexample}[1][]{\refstepcounter{counterexample}\par\medskip\indent%
\textbf{Counterexample~\thecounterexample #1}: \rmfamily}{\medskip}


% \newcounter{definition}
% \newenvironment{definition}[1][]% {\refstepcounter{definition}\par\medskip\indent%
% \textbf{Definition.} \rmfamily}{\medskip}
%\newcounter{definition}
%\newenvironment{definition}[1][]{\refstepcounter{definition}\par\medskip\indent%
%\textbf{Definition~\thedefinition #1}: \rmfamily}{\medskip}

% \newcounter{theorem}
% \newenvironment{theorem}[1][]{\refstepcounter{theorem}\par\medskip\noindent%
% \textbf{Theorem~\thetheorem #1}. \rmfamily}{\medskip}

% \newcounter{proposition}
% \newenvironment{proposition}[1][]{\refstepcounter{proposition}\par\medskip\indent%
% \textbf{Proposition~\theproposition #1}. \rmfamily}{\medskip}

% \newcounter{result}
% \newenvironment{result}[1][]{\refstepcounter{result}\par\medskip\indent%
% \textbf{Result~\theresult #1}. \rmfamily}{\medskip}

% \newcounter{proof}
% \newenvironment{proof}[1][]{\refstepcounter{proof}\par\medskip\noindent%
% \textbf{Proof.} \rmfamily}{\medskip}

\newcounter{tproof}
\setcounter{tproof}{0}
\newcommand{\tproof}{%
\addtocounter{tproof}{1}%
\paragraph{Proof of Theorem \arabic{theorem}.}}

\newcounter{corollary}
\newenvironment{corollary}[1][]{\refstepcounter{corollary}\par\medskip\indent%
\textbf{Corollary~\thecorollary #1}. \rmfamily}{\medskip}

\newcounter{cproof}
\setcounter{cproof}{0}
\newcommand{\cproof}{%
\addtocounter{cproof}{1}%
\paragraph{Proof of Corollary \arabic{corollary}.}}

% \newcounter{lemma}
% \newenvironment{lemma}[1][]{\refstepcounter{lemma}\par\medskip\noindent%
% \textbf{Lemma~\thelemma #1}. \rmfamily}{\medskip}

\newcounter{com}
\newenvironment{com}[1][]{\refstepcounter{com}\par\medskip\indent%
\textbf{Remark~\thecom #1}. \rmfamily}{\medskip}

\newcounter{lproof}
\setcounter{lproof}{0}
\newcommand{\lproof}{%
\addtocounter{lproof}{1}%
\paragraph{Proof of Lemma \arabic{lemma}.}}

%\newcounter{proof}
%\setcounter{proof}{0}
%\newcommand{\proof}{%
%\addtocounter{proof}{1}%
%\paragraph{Proof.}}

\newcounter{condition}
\newenvironment{condition}[1][]{\refstepcounter{condition}\par\medskip\noindent%
\textbf{Condition~\thecondition #1}. \rmfamily}{\medskip}

\newif\ifmydraft
%\mydrafttrue
\mydraftfalse

 \newcommand{\jl}[1]{\color{blue}{\small #1}\color{black}}
\ifmydraft
  \newcommand{\draftcolor}{purple}
  \pagecolor{black!20}
\else
  \newcommand{\draftcolor}{black}
\fi

\newcommand{\ms}[1]{\color{red}{\small #1}\color{black}}
\ifmydraft
  \newcommand{\draftcolor}{purple}
  \pagecolor{black!20}
\fi

\usepackage{multicol}
\newcommand{\indexlr}{{\textcolor{\draftcolor}{\ensuremath{k}}}}
\newcommand{\tuningparameter}{\textcolor{\draftcolor}{\ensuremath{\gamma}}}
\newcommand{\tuningparameterO}{\textcolor{\draftcolor}{\ensuremath{\tuningparameter^{\star}}}}
\newcommand{\tuningparameterAV}{\textcolor{\draftcolor}{\ensuremath{\gamma_D}}}
%\newcommand{\tuningparameterAV}{\textcolor{\draftcolor}{\ensuremath{\widetilde\delta}}}
\newcommand{\tuningparameterLB}{\textcolor{\draftcolor}{\ensuremath{\gamma_T}}}
\newcommand{\tuningparameterA}{\textcolor{\draftcolor}{\ensuremath{\delta}}}
\newcommand{\totalnumber}{\textcolor{\draftcolor}{\ensuremath{\binom{N}{2}}}}
\newcommand{\constre}{\textcolor{\draftcolor}{\ensuremath{C_{\operatorname{RE}}}}}
\newcommand{\consten}{\textcolor{\draftcolor}{\ensuremath{C}}}
\newcommand{\constsn}{\textcolor{\draftcolor}{\ensuremath{C_{\operatorname{T}}}}}
\newcommand{\constfn}{\textcolor{\draftcolor}{\ensuremath{C_{\operatorname{FN}}}}}
\newcommand{\dvalue}{\textcolor{\draftcolor}{\ensuremath{\mD}}}
\newcommand{\dvalueN}{\textcolor{\draftcolor}{\ensuremath{|\!|\!|\mD|\!|\!|_2}}}
\newcommand{\dvalueNsquare}{\textcolor{\draftcolor}{\ensuremath{|\!|\!|\mD|\!|\!|_2^2}}}
\newcommand{\threshold}{\textcolor{\draftcolor}{\ensuremath{\lambda}}}
\newcommand{\thresholdAV}{\textcolor{\draftcolor}{\ensuremath{\widetilde{\lambda}}}}
\newcommand{\smooth}{\textcolor{\draftcolor}{\ensuremath{\Psi}}}
\newcommand{\nbrsamples}{\textcolor{\draftcolor}{\ensuremath{N}}}
\newcommand{\nbrobservations}{\textcolor{\draftcolor}{\ensuremath{n}}}
\newcommand{\nbrparameters}{\textcolor{\draftcolor}{\ensuremath{p}}}
\newcommand{\nbrvertices}{\textcolor{\draftcolor}{\ensuremath{M}}}
\newcommand{\parameterE}{\textcolor{\draftcolor}{\ensuremath{\theta}}}
\newcommand{\parameter}{\textcolor{\draftcolor}{\ensuremath{\boldsymbol{\parameterE}}}}
\newcommand{\parameterT}{\textcolor{\draftcolor}{\ensuremath{\parameter^\star}}}
\newcommand{\parameterTT}{\textcolor{\draftcolor}{\ensuremath{\parameter_{\settrue}^\star}}}
\newcommand{\parameterTF}{\textcolor{\draftcolor}{\ensuremath{\parameter_{\settrueC}^\star}}}
\newcommand{\parameterTE}{\textcolor{\draftcolor}{\ensuremath{\parameterE^\star}}}
\newcommand{\parameterTj}{\textcolor{\draftcolor}{\ensuremath{\parameterE_k^\star}}}
\newcommand{\parameterj}{\textcolor{\draftcolor}{\ensuremath{\parameterE_k}}}
\newcommand{\parameterTGj}{\textcolor{\draftcolor}{\ensuremath{\parameter_{\groupj}^\star}}}
\newcommand{\parameterTi}{\textcolor{\draftcolor}{\ensuremath{\theta_i^\star}}}
\newcommand{\parameterTS}{\textcolor{\draftcolor}{\ensuremath{\parameter_{\mathcal{S}^\star}^\star}}}
\newcommand{\parameterspace}{\textcolor{\draftcolor}{\ensuremath{\boldsymbol{\Theta}}}}
\newcommand{\estimator}{\textcolor{\draftcolor}{\ensuremath{\widehat\parameter}}}
\newcommand{\destimator}{\textcolor{\draftcolor}{\ensuremath{\widehat\parameter}}}
\newcommand{\Destimator}{\textcolor{\draftcolor}{\ensuremath{\widehat\parameterspace}}}
\newcommand{\Estimator}{\textcolor{\draftcolor}{\ensuremath{\widehat\parameterspace}}}
\newcommand{\estimatorAV}{\textcolor{\draftcolor}{\ensuremath{\widetilde\parameter}}}
\newcommand{\estimatorAVE}{\textcolor{\draftcolor}{\ensuremath{\widetilde\parameterE}}}
\newcommand{\estimatorj}{\textcolor{\draftcolor}{\ensuremath{\widehat\theta_j}}}
\newcommand{\estimatorT}{\textcolor{\draftcolor}{\ensuremath{\widetilde{\parameter}}}}
\newcommand{\estimatorE}{\textcolor{\draftcolor}{\ensuremath{\widehat\parameterE}}}
\newcommand{\estimatorTE}{\textcolor{\draftcolor}{\ensuremath{\widetilde{\parameterE}}}}
\newcommand{\settrue}{\textcolor{\draftcolor}{\ensuremath{\mathcal{S}^\star}}}
\newcommand{\estimatorSupp}{\textcolor{\draftcolor}{\ensuremath{\widehat{\mathcal{S}}}}}
\newcommand{\estimatorSuppAV}{\textcolor{\draftcolor}{\ensuremath{\widehat{\mathcal{S}}(\tuningparameterAV)}}}
%\newcommand{\levelre}{\textcolor{\draftcolor}{\ensuremath{t_{\operatorname{RE}}}}}
\newcommand{\levelre}{\textcolor{\draftcolor}{\ensuremath{u}}}
%\newcommand{\levelen}{\textcolor{\draftcolor}{\ensuremath{t_{\operatorname{EN}}}}}
\newcommand{\levelen}{\textcolor{\draftcolor}{\ensuremath{t}}}
\newcommand{\goodevent}{\textcolor{\draftcolor}{\ensuremath{\mathcal{E}}}}

\newcommand{\avconst}{\textcolor{\draftcolor}{\ensuremath{L}}}

\newcommand{\su}{\sup\limits}
\newcommand{\bg}{\bm{g}}
\newcommand{\reS}{\textcolor{\draftcolor}{\ensuremath{\Lambda}}}
\newcommand{\re}{\textcolor{\draftcolor}{\ensuremath{\reS}}}
\newcommand{\fn}{\textcolor{\draftcolor}{\ensuremath{C_{\operatorname{FE}}}}}
\newcommand{\last}{\textcolor{\draftcolor}{\ensuremath{C_3}}}
\newcommand{\settrueC}{\textcolor{\draftcolor}{\ensuremath{\overline{\mathcal{S}}^{\star}}}}
\newcommand{\gradA}{\textcolor{\draftcolor}{\ensuremath{\nabla_{\parameter}}\;}}
\newcommand{\gradAj}{\textcolor{\draftcolor}{\ensuremath{\nabla_{\parameter_{\groupj}}}\;\,}}
\newcommand{\loss}{\textcolor{\draftcolor}{\ensuremath{\ell}}}
\newcommand{\lossP}{\textcolor{\draftcolor}{\ensuremath{\widetilde\loss}}}
\newcommand{\dataE}{\textcolor{\draftcolor}{\ensuremath{Y}}}
\newcommand{\dataEs}{\textcolor{\draftcolor}{\ensuremath{y}}}
\newcommand{\datab}{\textcolor{\draftcolor}{\ensuremath{\boldsymbol{y}}}}
\newcommand{\covar}{\textcolor{\draftcolor}{\ensuremath{\boldsymbol{X}}}}
\newcommand{\data}{\textcolor{\draftcolor}{\ensuremath{\boldsymbol{\dataE}}}}
\newcommand{\lossPA}{\textcolor{\draftcolor}{\ensuremath{\lossP(\parameter;\, \covar,\, \data)}}}
\newcommand{\sufficient}{\textcolor{\draftcolor}{\ensuremath{s}}}
\newcommand{\design}{\textcolor{\draftcolor}{\ensuremath{\bX}}}
\newcommand{\designV}{\textcolor{\draftcolor}{\ensuremath{\boldsymbol{x}}}}
\newcommand{\noiseE}{\textcolor{\draftcolor}{\ensuremath{\bm\epsilon}}}
\newcommand{\noise}{\textcolor{\draftcolor}{\ensuremath{\boldsymbol{\noiseE}}}}
\newcommand{\norm}[1]{\lVert#1\rVert}
\renewcommand{\norm}[1]{|\!|#1|\!|}
\newcommand{\normB}[1]{\big|\!\big|#1\big|\!\big|}
\newcommand{\normBB}[1]{\Big|\!\Big|#1\Big|\!\Big|}
\newcommand{\normBBB}[1]{\bigg|\!\bigg|#1\bigg|\!\bigg|}
\newcommand{\normBBBB}[1]{\Bigg|\!\Bigg|#1\Bigg|\!\Bigg|}
\newcommand{\normone}[1]{\norm{#1}_1}
\newcommand{\normsup}[1]{\norm{#1}_{\infty}}
\newcommand{\normsupB}[1]{\normB{#1}_{\infty}}
\newcommand{\normsupBB}[1]{\normBB{#1}_{\infty}}
\newcommand{\normsupBBB}[1]{\normBBB{#1}_{\infty}}
\newcommand{\normsupBBBB}[1]{\normBBBB{#1}_{\infty}}
\newcommand{\normtwo}[1]{\norm{#1}_2}
\newcommand{\normGone}[1]{\norm{#1}_{1,2}}
\newcommand{\normGsup}[1]{\norm{#1}_{\infty,2}}
\newcommand{\normGsupB}[1]{\normB{#1}_{\infty,2}}
\newcommand{\normGsupBB}[1]{\normBB{#1}_{\infty,2}}
\newcommand{\normGsupBBB}[1]{\normBBB{#1}_{\infty,2}}
\makeatletter
\newcommand*{\deq}{\mathrel{\rlap{%
  \raisebox{0.3ex}{$\m@th\cdot$}}%
  \raisebox{-0.3ex}{$\m@th\cdot$}}=}
\makeatother
\newcommand{\tp}{^\top}

\newcommand{\group}{\textcolor{\draftcolor}{\ensuremath{\mathcal{A}}}}
\newcommand{\groupj}{\textcolor{\draftcolor}{\ensuremath{\group_g}}}
\newcommand{\nbrgroups}{\textcolor{\draftcolor}{\ensuremath{G}}}
%\newcommand{\sizegroups}{\textcolor{\draftcolor}{\ensuremath{\max_{1 \leq g \leq \nbrgroups}}}}



==> old.test.simulations.tex <==
To simulate data,
there are at least two possible approaches.
For ease of presentation,
we focus on simulating treatment assignments and potential outcomes,
and assume that the interference graph is known.

\vspace{.05cm}

{\em Fixed potential outcomes:}
For each of the $2^N$ possible treatment assignments $\bx \in \{0, 1\}^N$,
specify the $N$ potential outcomes $\by(\bx)$ by specifying a function of $\bx$ and evaluating it.
Then generate one of the treatment assignments $\bx \in \{0, 1\}^N$ at random and call the result $\bx^{obs}$.
The $N$ observed outcomes are then $\by^{obs} = \by(\bx^{obs})$.

\vspace{.05cm}

{\em Random potential outcomes:}
For each of the $2^N$ possible treatment assignments $\bx \in \{0, 1\}^N$,
generate the $N$ potential outcomes by specifying a joint probability law for $\bY(\bx)$ and generating a realization $\by(\bx)$ of $\bY(\bx)$.
Then generate one of the treatment assignments $\bx \in \{0, 1\}^N$ at random,
independent of the set of potential outcomes $\{\by(\bx):\; \bx \in \{0, 1\}^N\}$,
and call the result $\bx^{obs}$.
The $N$ observed outcomes are then $\by^{obs} = \by(\bx^{obs})$.

\vspace{.05cm}

To assess the tests described in Section \ref{sec:conditional.randomization.test.interference},
we do not need to generate the potential outcomes $\by(\bx)$ for any $\bx \neq \bx^{obs}$:
all we need to compute $p$-values is $\bx^{obs}$ and $\by^{obs} = \by(\bx^{obs})$.
So we can generate first $\bx^{obs}$ and then $\by^{obs}$.
Given $\bx^{obs}$ and $\by^{obs}$ along with a test statistic $T_{\mathscr{U},\mathscr{V}}(\bX, \by^{obs})$,
we can calculate the $p$-value $p(\bx^{obs})$ based on the probability distribution of $\bX \mid \mU, \bX \in \mV$.

\vspace{.05cm}

Since the test procedure does not make any assumptions about the process generating potential outcomes,
either the fixed or the random potential outcome approach can be used to simulate data.
We use the random approach because it is convenient and consistent with common practice in statistics and data science.
We generate 1,000 data sets with $N = 500$ and $N = $ 1,000 units,
with treatment assignments $\bX$ generated from
\beno
\mbP_{\mX}(\bX = \bx)
&=& \dfrac{1}{\binom{N}{M}}\ \text{for all }\bx\text{ such that}\ \dsum_{i=1}^{N} x_i = M,
\ee
where $M \coloneqq 2\, N / 5$. 
The interference graph $\bZ$ is generated by a rank-one random graph model \citep{latent.space.models.theory}:
\beno 
Z_{i,j} 
&\ind& \text{Bernoulli}(P_{i,j}),\;
& 
P_{i,j} 
&\coloneqq& \alpha_i\, \alpha_j,\;
& \alpha_i\, \iid\, \mbox{Beta}(1,\, 3).
\ee
% Subhankar: It is important to specify what all potential outcomes are. Otherwise, the framework is unclear.
% Note that in our simulation study, we are not working with one x^{obs}. For each replication i, we are getting a new x^{obs, i}. Then we are generating the observed outcomes for the i-th replication y^{obs,i} from a multivariate Gaussian.
% That is justified because we have assumed all potential outcomes are realizations from Gaussian.
% I think we should keep this narrative. This is not clear from the previous paragraph. I have changed the following paragraph accordingly. I would request to not delete major changes entirely. 
We assume that the potential outcomes $y_i(\bx)$ ($\bx\in\mX$) are realizations from a multivariate Gaussian.
The multivariate Gaussian has conditional distributions  % with conditional expectations of\,
$Y_i(\bx) \mid (\bY_{-i}(\bx), \bZ) = (\by_{-i}(\bx), \bz^{obs})$ with expectations stated in Section \ref{sec:characterizing.causal.effects},
with scaling constants $c_{N,i,1}(\bz^{obs}) = 1/\sum_{j=1}^N\, z_{i,j}^{obs}$ and $c_{N,i,2}(\bz^{obs})=1/\mnorm{\bz^{obs}}_2$,
 and conditional variance $1$.
This multivariate Gaussian can be shown to capture spillover along with statistical dependence among potential outcomes $Y_1(\bx), \ldots, Y_N(\bx)$ induced by contagion.
Based on the generated treatment assignments $\bx^{obs}$, 
we generate the potential outcomes $\by(\bx^{obs})=\by^{obs}$ from a multivariate Gaussian with conditional expectations stated in Section \ref{sec:characterizing.causal.effects};
note that the potential outcomes $\by(\bx)$ corresponding to treatment assignments $\bx \neq \bx^{obs}$ are not required,
so we do not generate them.
We then select $30\%$ of the observations at random and use them as focal units $\mathscr{U}$..
We then evaluate interference using the test statistic $T_{\mathscr{U},\mathscr{V}}(\bX, \by_\mathscr{U}^{obs})$ in Equation \eqref{athey} and compute the $p$-value $p(\bx^{obs})$ in Equation \eqref{p.value} under the probability distribution of $\bX\mid \mU,\bX\in\mV$. .
The simulation results can be interpreted as randomization tests performed in a fixed potential outcome framework,
where the set of fixed potential outcomes $\{\by(\bx):\; $ ($\bx \in \mX\}$) is generated from are realizations from a multivariate Gaussian.
% We denote the generated treatment assignments and interference graph by $\bx^{obs}$ and $\bz^{obs}$,
% respectively.
% We then generate $\by^{obs} = \by(\bx^{obs})$ by generating a realization $\by(\bx^{obs})$ from a multivariate Gaussian.
% The multivariate Gaussian has conditional distributions $Y_i(\bx^{obs}) \mid (\bY_{-i}(\bx^{obs}), \bZ) = (\by_{-i}(\bx^{obs}), \bz^{obs})$ with expectations stated in Section \ref{sec:characterizing.causal.effects},
% scaling constants $c_{N,i,1}(\bz^{obs}) = 1/\sum_{j=1}^N\, z_{i,j}^{obs}$ and $c_{N,i,2}(\bz^{obs})=1/\mnorm{\bz^{obs}}_2$,
% and conditional variance $1$.
% This multivariate Gaussian can be shown to capture spillover along with statistical dependence among potential outcomes $Y_1(\bx^{obs}), \ldots, Y_N(\bx^{obs})$ induced by contagion.
% We select $30\%$ of the observations at random and use them as focal units $\mathscr{U}$.
% We then evaluate the test statistic $T_{\mathscr{U},\mathscr{V}}(\bX, \by_\mathscr{U}^{obs})$ in Equation \eqref{athey} and compute the $p$-value $p(\bx^{obs})$ in Equation \eqref{p.value} under the probability distribution of $\bX\mid \mU,\bX\in\mV$. 
% The simulation results can be interpreted as randomization tests performed in a fixed potential outcome framework,
% where the set of potential outcomes $\{\by(\bx):\; \bx \in \mX\}$ is generated from a multivariate Gaussian.

==> partial_interference.tex <==
\begin{appendix}

\section{Spillover in subpopulations}

%\alert{I wonder whether we discuss the classic work of \citet{HuHa08} in too much detail. We may have to be selective.}

%\sbh{Subhankar: I agree.}

\citet{HuHa08} were among the first to formally study causal inference under interference.
\citeauthor{HuHa08} considered a two-stage randomization framework,
assuming that the population of interest is partitioned into $K \geq 2$ subpopulations,
called blocks.
In the first stage, two treatment assignment strategies of interest, say $\alpha_0$ and $\alpha_1$, are randomly allotted to the $K$ blocks via some randomization strategy $\nu$.
Next, within each block, the treatment $X$ is assigned to the units according to the corresponding assignment strategy.
It is assumed that interference is allowed to happen only within units in the same block.
Let $S_k$ be the indicator that the $k$-th block was assigned $\alpha_1$ and $N_k$ be the size of the $k$-th block, $k=1,2,\ldots,K$.
Let $b_i$ be the block the $i$-th unit belongs to, and let $\mcN_i$ be the set of all units in it except $i$.
%, that is, $$\mcN_i\; =\; \{j:b_j = b_i,\; j\neq i\}.$$
Let $\bx_{-i}$ be the set of treatments assigned to the neighbors of $i$, 
i.e.,
$$\bx_{-i}\coloneqq\{x_j:j\in\mcN_i\}.$$ 
Then in their setting, the $i$-th potential outcome can be written as $Y_i(x_i;\bX_{-i})$. 
\citeauthor{HuHa08} also assumed a finite population, 
i.e., 
the potential outcomes are fixed.
%For $i\neq j$, let $A_{i,j}$ be the indicator if two units $i$ and $j$ are in the same block, and let $A_{i,i}=0$.
%let $\mcN_i$ be the set of all units in it except $i$, that is,
%$$\mcN_i=\{j:A_{i,j} = 1\}.$$

In the two-stage randomization setting, \citet{HuHa08} defined four causal estimands that can be of interest: direct effect, indirect effect, total effect, and overall effect.
We define these causal effects below.

First, 
let us define $\bar{Y}_i(x,\alpha_s)$ to be the expected potential outcome of the $i$-th unit conditioned on the event that treatment level $x$ was assigned to it, under the law of $\alpha_s$, 
i.e.,
\begin{equation}
    \bar{Y}_i(x,\alpha_s)\coloneqq \mbE_{\mathscr{X}}i{\alpha_s}{x}[Y_i(x;\bX_{-i})].
\end{equation}

\hide{

\alert{{How about replacing $\bar{Y}_i(x,\phi)$ and $\bar{Y}_i(x,\psi)$ by the following expectations?}
\begin{equation}
\dint Y_i(x,\, \bX_{-i}) \dd \mbP_0,
\end{equation}
{and}
\begin{equation}
\dint Y_i(x,\, \bX_{-i}) \dd \mbP_1,
\end{equation}
{where $\mbP_0$ and $\mbP_1$ are the probability measure corresponding to $\phi$ and $\psi$. 
As mentioned before, it would help streamline notation throughout the paper.}
}

\sbh{Subhankar: The expectations are conditional on $X_i = 0$ or 1. They assume a mixed assignment strategy which makes treatment assignments dependent because the sum is fixed. The alternative is Bernoulli assignment strategy, which gives us independence, e.g. in Li and Wager. We need to define both of them somewhere. HH08 and TV12 have defined mixed assignment strategy, but I am trying to write it in a concise way without introducing many notations.}

}

The direct effect captures the effect of the treatment assigned to a unit on its expected potential outcome.
%The block-level estimands are only interesting when we have disjoint blocks, whereas the population-level estimands
The {block average direct effect} (for assignment strategy $\alpha_s$) is defined as
\begin{align*}
    \bar{DE}_k(\alpha_s)=\frac{1}{N_k}\sum_{i\,:\,b_i=k}(\bar{Y}_i(1,\alpha_s) - \bar{Y}_i(0,\alpha_s)),
\end{align*}
for $s=0,1;\,k=1,\ldots, K$. 
We see that under no interference, $\bar{DE}_k(\alpha_s)$ becomes equal to the average treatment effect for the $k$-th block, which we defined in \eqref{ate}.
The {population average direct effect} is simply the average of the block-level direct effects $\bar{DE}(\alpha_s) = 1/K\sum_{k=1}^K\bar{DE}_k(\alpha_s)$.

Next, the indirect effect is intended to capture the effect on the potential outcome of a unit of the treatments assigned to other units in its block, holding the treatment assigned to it at a fixed level, say 0.
The {block average indirect effect} is defined as
\begin{align*}
    \bar{IE}_k(\alpha_0,\alpha_1)=\frac{1}{N_k}\sum_{i\,:\,b_i=k}(\bar{Y}_i(0,\alpha_1) - \bar{Y}_i(0,\alpha_0)),
\end{align*}
for $k=1,\ldots, K$. 
The total effect reflects both the direct and indirect effects of the treatment assignment scheme on the potential outcomes. The {block average total effect} is
\begin{align*}
    \bar{TE}_k(\alpha_0,\alpha_1)=\frac{1}{N_k}\sum_{i\,:\,b_i=k}(\bar{Y}_i(1,\alpha_1) - \bar{Y}_i(0,\alpha_0)),
\end{align*}
for $k=1,\ldots, K$. Finally, the overall effect captures the effect of the treatment assignment scheme on the potential outcomes.
The {block average overall effect} is
\begin{align*}
    \bar{OE}_k(\alpha_0,\alpha_1)=\frac{1}{N_k}\sum_{i\,:\,b_i=k}(&\,\mathbb{E}_{{\mathbb{P}_{\alpha_1}}_{(X_i,\bX_{-i})}}Y_i(X_i;\bX_{-i})\, - \\
    &\,\mathbb{E}_{{\mathbb{P}_{\alpha_0}}_{(X_i,\bX_{-i})}}Y_i(X_i;\bX_{-i})).
\end{align*}
As we defined for the direct effect, the population-level effects $\bar{IE}(\alpha_0,\alpha_1),\bar{TE}(\alpha_0,\alpha_1)$ and $\bar{OE}(\alpha_0,\alpha_1)$ are defined as the averages of the corresponding block-level effects.

\citet{HuHa08} proposed unbiased estimators for all of the four effects at the population level. 
To discuss the estimators, let us first define the quantity
$$
\mu_k(x,\alpha_s)\; \coloneqq\; \frac{1}{N_k}\sum_{i\,:\,b_i=k}\bar{Y}_i(x,\alpha_s).
$$
$\mu_k(x,\alpha_s)$ is the average of the expected potential outcomes of units in the $k$-th block, under assignment strategy $\alpha_s$.
The authors showed that if $\alpha_0$ and $\alpha_1$ are mixed assignment strategies and $S_k=s$, then an unbiased estimator of 
$\mu_k(x,\alpha_s)$ is given by,
$$\widehat{\mu}_k(x)\; \coloneqq\; \frac{\sum_{i\,:\,b_i=k}Y_i\,\mbI(X_i=x)}{\sum_{i\,:\,b_i=k}\mbI(X_i=x)}.$$
Now observe that the first three of the causal effects, namely, the direct, indirect, and total effect, are functions of $\mu_k(x,\alpha_s)$.
Therefore, given that $S_k=s$, the block average direct effect $\bar{DE}_k(\alpha_s)$ is estimated by $\widehat{\mu}_k(1) - \widehat{\mu}_k(0)$.
Unfortunately, since only one of $\alpha_0$ and $\alpha_1$ will be assigned to a particular block, it is not possible to estimate the other effects at the block level.
At the population level, the authors showed that if the randomization $\nu$ in the first stage is again a mixed assignment strategy, then an unbiased estimator of $1/K\sum_{k=1}^K\mu_k(x,\alpha_s)$ is given by $\sum_{k=1}^K\widehat\mu_k(x)\,\mbI(S_k=s)/\sum_{k=1}^K\mbI(S_k=s)$.
Based on this, we can have unbiased estimators of the population-level effects $\bar{DE}(\alpha_s),\bar{IE}(\alpha_0,\alpha_1)$ and $\bar{TE}(\alpha_0,\alpha_1)$.
For the overall effect, similar types of calculations show that an unbiased estimator of $\bar{OE}(\alpha_0,\alpha_1)$ is
\begin{align*}
    &\,\frac{\sum_{k=1}^K\left(\frac{1}{N_k}\sum_{i\,:\,b_i=k}Y_i\right)\mbI(S_k=1)}{\sum_{k=1}^K\mbI(S_k=1)}\, - \\
    &\,\frac{\sum_{k=1}^K\left(\frac{1}{N_k}\sum_{i\,:\,b_i=k}Y_i\right)\mbI(S_k=0)}{\sum_{k=1}^K\mbI(S_k=0)}.
\end{align*}

While proposing unbiased estimators for the causal effects is an important step, a more challenging aspect under interference is to ensure the precision and consistency of the estimators, as has been pointed out in recent papers such as \cite{savje2021average, LiWa22}.
\citet{HuHa08} also proposed estimators of the variances of the estimators discussed above under an assumption called {stratified interference}.
\begin{assumption}
    {\em Stratified interference.} The potential outcome of a unit $i$ depends on the treatments assigned to the neighbors of $i$ only via the number of units that received treatment level 1 (or 0). Mathematically,
    \begin{gather*}
        Y_i(x_i;\bX_{-i})=Y_i(x'_i;\bx'_{-i})\\
        \text{if}\ x_i=x'_i\ \text{and}\ \sum_{j\in \mcN_i}x_j = \sum_{j\in \mcN_i}x'_j.
    \end{gather*}
\end{assumption}

\vspace{-.5cm}
\noindent
Under stratified interference, the authors gave unbiased estimators for $\mbox{Var}(\widehat\mu_k(x)|S_k=s)$ and based on them, proposed estimators for the variances of the causal effect estimators.
We refer readers to \cite{HuHa08} for details.

\sbh{Important comment about how this reduces the missing data problem of observing $N$ of $\sim2^N$ to observing $N$ of $4N$ many potential outcomes.
So, the difficulty is sort of in the same level as the no interference case, where the missing data problem is that we observe $N$ out of $2N$ many potential outcomes.
However, this simplification only happens under subpopulation structure, and, with mixed assignment strategy.
For a general network, stratified interference is still a hard problem.}

%Assumption 1 has been found crucial for inference under interference in several subsequent papers \cite{Ogetal20, savje2021average,LiWa22}.
\citet{tchetgen2012causal} proposed more conservative estimators for $\mbox{Var}(\widehat\mu_k(x)|S_k=s)$ without requiring Assumption 1, 
but assumed that all the potential outcomes are non-negative.
\citeauthor{tchetgen2012causal} also derived finite-sample confidence intervals of the population-level causal effects in the case when the potential outcomes are binary, using Hoeffding-type exponential inequalities.
Following that, \citet{rigdon2015exact} proposed new finite-sample confidence sets, again for the binary case, that were empirically shown to be much narrower than the confidence interval proposed in \cite{tchetgen2012causal}.
In their method, we consider the set $\mY$ of all possible potential outcome vectors that are compatible with the observed outcomes.
For each vector in $\mY$, we test if the causal effect of interest, say the direct effect, is equal to the direct effect value uniquely determined by the potential outcome vector.
Then the confidence set for the direct effect is given by all the direct effect values for which the $p$-value of the test is large enough (depending on confidence level). 
Of course, the downside of this method is that it can be computationally very expensive when $N$ is large.
\citet{liu2014large} derived asymptotic distribution of the causal effect estimators under two regimes: (i) when sizes of the subpopulations, $\min_k N_k\rightarrow \infty$, (ii) when the number of subpopulations, $K\rightarrow\infty$. For both cases, the causal effect estimators were shown to converge to the normal distribution under certain homogeneity conditions.
The asymptotic results were then used to construct Wald-type confidence intervals for the causal effects.

\sbh{Pausing this subsection here.\\
Other interesting and cited works: \citet{tchetgen2012causal} and \citet{liu2016inverse} discuss IPW estimators which are relevant for observational studies, when one can not control the assignment mechanism, and it is typically assumed that the assignment probabilities depend on some covariate $L_i$.
These two papers also discussed Bernoulli assignment instead of mixed assignment.

\citet{basse2018analyzing} (2018) discusses the problem of assigning equal probability to households (blocks).
\citet{baird2018optimal} discusses optimally designing the two-stage experiments (choosing the parameters).}
%Most of the literature on this topic considered this population interference graph to be fixed or non-random, which we discuss in Section \ref{subsec:fixed}.
%Next, in Section \ref{subsec:random}, we discuss the case when the population interference graph is considered random.

\end{appendix}

==> test.violation.tex <==
The low power of the test for detecting interference arising from contagion may stem from a combination of two issues:
\bi 
\item the test statistic $T_{\mathscr{U},\mathscr{V}}(\bX, \by_{\mathscr{U}}^{obs})$ in Equation \eqref{athey} is designed to capture interference via neighbors,
but contagion allows the potential outcomes of unit $i$ to be affected by the treatment assignments $x_j$ of non-neighbors $j$ via their potential outcomes $y_j(\bx)$;
\vspace{.05cm}
\item the strength of interference decays as a function of geodesic distance in the interference graph,
where the geodesic distance between two units $i$ and $j$ is the length of the shortest path between them \citep{leung2022rate}.
\ei 
We demonstrate violations of neighborhood exposure assumptions in Figures \ref{fig:con.pop} and \ref{graph.exposure} in Section \ref{assumption1}.

==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
\tikzstyle{alive} = [latent,fill=black]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


